Understanding and Leveraging the Learning Phases of Neural Networks

The learning dynamics of deep neural networks are not well understood. The information bottleneck (IB) theory proclaimed separate fitting and compression phases. But they have since been heavily debated. We comprehensively analyze the learning dynamics by investigating a layer's reconstruction ability of the input and prediction performance based on the evolution of parameters during training. We empirically show the existence of three phases using common datasets and architectures such as ResNet and VGG: (i) near constant reconstruction loss, (ii) decrease, and (iii) increase. We also derive an empirically grounded data model and prove the existence of phases for single-layer networks. Technically, our approach leverages classical complexity analysis. It differs from IB by relying on measuring reconstruction loss rather than information theoretic measures to relate information of intermediate layers and inputs. Our work implies a new best practice for transfer learning: We show empirically that the pre-training of a classifier should stop well before its performance is optimal.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> toadd_15.tex <==
\begin{abstract}
The learning dynamics of deep neural networks are not yet understood. The information bottleneck (IB) theory proclaimed separate fitting and compression phases. But they have since been heavily debated. We contribute a rigorous analysis of the learning dynamics by analyzing a layer's reconstruction ability of the input and prediction performance based on the evolution of parameters during training. We show the existences of three phases using common datasets and architectures from computer vision such as ResNet and VGG: near constant reconstruction loss, decrease and increase in empirical settings. We also theoretically proclaim two data configurations and show theoretically for single layer networks that under these configurations the phases must exist. The first configuration is built on the observation that data can exist with features of various strengths. The second setting captures the observation that the majority of samples might initially dominate learning, leading the classifier to learn prototypical instances (averages). But at a later stage a few samples can cause learning to shift, potentially, undoing initial learning for the majority of samples. That is, majority samples might by classified using only a (small) subset of the priorly learnt features. Technically, our approach differs from IB by relying on measuring reconstruction loss rather than information theoretic measures to relate information of intermediate layers and inputs.  
\end{abstract}

\section{Introduction}
Deep neural networks are arguably the key driver of the current boom in artificial intelligence(AI) in academia and industry. They achieve superior performance in a variety of domains. Still, they suffer from poor understanding, which has even led to an entire branch of research, i.e., explainability(XAI)~\citep{mesk22}, and to widespread debates on trust in AI within society. Thus, enhancing our understanding of how deep neural networks work is arguably one of key problems in ongoing machine learning research~\citep{pog20}. Unfortunately, the relatively few theoretical findings and reasonings are often subject to rich controversy. 

One debate surrounds the core of machine learning: learning behavior. ~\citet{tish17} leveraged the information bottleneck(IB) framework to investigate the learning dynamics of neural networks. IB relies on measuring mutual information between activations of a hidden layer and the input as well as the output. A key qualitative, experimental finding was the existence of a fitting and compression phase during the training process. Compression is conjectured a reason for good generalization performance. It is frequently discussed in the literature~\citep{gei21,jak19}. Such a finding can be considered a breakthrough result in the understanding of deep neural networks. However, its validity has been disputed, i.e., Saxe et al.~\citep{saxe19} claimed that statements in~\citep{tish17} do not generalize to common activation functions. Today, the debate is still ongoing~\citep{lor21}. A key challenge is the difficulty in approximating the IB. This, makes a rigorous mathematical treatment very hard -- even empirical analysis is non-trivial.\\

In this work, we also aim to study the learning behavior with a focus on fitting and compression capability of layers but propose a different lens for investigation. We aim to perform a rigorous analysis of a linear classifier and a model of the data built on empirical evidence. In contrast to prior work relying only on general statements that lack mathematical proof, we provide a show bounds on the duration of (some) phases highlighting interplays, e.g., between the number of samples, the number of classes and the number of input attributes. Such behavior were not considered in prior work based on IB. 
Second, we utilize different measures from IB. Rather than measuring the information a layer provides on an output~\citep{tish17}, we measure how well the layer can be used to classify samples (as in~\citep{ala17}, when a simple classifier is trained on the layer activations, i.e., we investigate linear separability of classes given layer activations.  
Rather than measuring the information of a layer with respect to the input~\citep{tish17}, we measure the reconstruction error of the input given the layer by utilizing a decoder.
Third, we provide two different data configurations and prove for single layer networks, i.e., linear networks, that they can both cause the three learning phases. In the first configuration, we show that the reconstruction error is likely to decrease early in the training, since the network essentially learns the class average, often resembling a prototype. The error increases later during training, if a classifier shifts from fitting the majority to fitting the (remaining) high loss samples. In this phase, the network might change from using non-noisy features to noisy features or simply rely on fewer features to reconstruct the majority of samples. In the second, we show that if samples of one class vary in strength, e.g., for images brightness of pixels can vary, such phases can also happen.  \\
%We also show empirically that such a behavior is common for multiple classifiers, datasets and layers.\\
The paper begins with an empirical analysis showing that such a behavior is common for multiple classifiers, datasets and layers followed by a theoretical analysis drawing on our empirical findings to model the problem and rigorously analyze a linear multi-class model. Finally, we state related work, discuss our work, especially limitations and generalization, and conclude.





% \begin{figure}[!htb]
% \centering{\centerline{\includegraphics[width=0.45\textwidth]{Lay0Fash_F0.png}} %\columnwidth
% \caption{Normalized accuracy and reconstruction loss for the F0 classifier and the FashionMNIST dataset} \label{fig:metF0Fa}}
% \end{figure}

% \begin{figure}[!htb]
% \centering{\centerline{\includegraphics[width=0.35\textwidth]{WeiFash_0_Cl5.png}} %\columnwidth
% %\vspace{-12pt}
% \caption{Weight matrices for the F0 classifier for each class across training for FashionMNIST\scriptsize{We showed only every 2nd to save space} }
% \label{fig:weiFa}}
% %\vspace{-12pt}
% \end{figure}

\section{Empirical analysis}
For a model $M=(L_0,L_1,...)$ consisting of a sequence of layers $L_i$, we discuss behavior of train and test accuracy for a linear classifier $CL$ trained on layer activations $L_i$ of model $M^{(t)}$ at different iterations $t$ during training. We also investigate the reconstruction loss of inputs using a decoder $DE$ to reconstruct inputs $X$ from layer activations $L_i$. %We employ multiple datasets, networks and layers. 
%$||X-\hat{X}||^2$ yielding an estimate $\hat{X}$ 


\subsection{Measures}
We assess outputs of each layer with respect to their ability to predict the output and reconstruct the input. %Intuitively, this relates to prior work~\citep{tish17} that aimed to capture the amount of information on the input and the output for a given layer.
To compute our measures for a model $M^{(t)}$ trained for $t$ iterations, we train two auxiliary models, i.e. a classifier $CL$ and a decoder $DE$. To assess prediction capability $Acc^{(t)}$ at iteration $t$ of the training, we use a simple dense layer as classifier $CL$ taking as input the outputs $L(X)$ of a layer $L \in M$. In this way, we assess to what extent the outputs $L(X)$ allow us to predict the correct class without much further transformation. %It predicts the class $Y$.

To obtain the reconstruction error $Rec^{(t)}$, we use a decoder $DE$ that takes as input the outputs $L(X)$ of a layer $L \in M$ and computes the estimate $\hat{X}$ yielding an error $||\hat{X}-X||^2$. 

Both auxiliary models are trained on $L(X)$ for all training data. The metrics $Acc^{(t)}, Rec^{(t)}$ are computed on the test data.


% \begin{figure*}[!htb]
% \centering{
% \centerline{\includegraphics[width=0.8\textwidth]{lotClFashSamp0.png}} %\columnwidth
% %\vspace{-12pt}
% \caption{Samples from FashionMNIST close to mean (left), far from mean with low dot product with mean (middle) and with large dot product (right) for the F0 classifier} \label{fig:loClFaSa}}
% %\vspace{-12pt}
% \end{figure*}

% \begin{figure*}[!htb]
% \centering{ \centerline{\includegraphics[width=0.9\textwidth]{lotClFash.png}} %\columnwidth
% %\vspace{-12pt}
% \caption{Loss for 1000 samples closest to the mean, samples furthest from the mean with smallest and largest dot product with the mean for FashionMNIST} \label{fig:loClFa} }
% %\vspace{-12pt}
% \end{figure*}

\subsection{Dataset, networks and setup} \label{sec:dat}
As networks for model $M$ we used VGG-11~\citep{sim14}, Resnet-10~\citep{he16} and fully connected networks, i.e., we employed networks $F0$ and $F1$, where the number denotes the number of hidden layers. A hidden layer has 256 neurons. After each hidden layer we applied the ReLU activation and batch-normalization. We used a fixed learning rate of 0.002 and stochastic gradient descent with batches of size 128 training for 256 epochs.  

We computed evaluation metrics $Acc^{(t)}$, $Rec^{(t)}$ at iterations $2^i$, i.e., $0,1,2,4,8...$.
For the decoder $DE$ we used the same decoder architecture as in~\citep{sch21cla}, where a decoder from a (standard) auto-encoder was used.  For each computation of the metrics, we trained the decoder for 30 epochs using the Adam optimizer with learning rate of 0.0003. For the classifier $CL$ we used a single dense layer trained using SGD with fixed learning rate of 0.003 for 20 epochs.
We used CIFAR-10/100~\citep{kri09}, Fashion-MNIST~\citep{xia17} and MNIST, all scaled to 32x32, available under the MIT (first 3 datasets) and GNU 3.0 licence. We trained each model $M$ 5 times. All figures show standard deviations. We report normalized metrics to better compare $Acc^{(t)}$ and $Rec^{(t)}$.


\subsection{Results}

%This is expected though for even longer training, we might observe overfitting, i.e., a decrease in test accuracy. This behavior is non-obvious.  though for classes with diverse samples this is not necessarily the case
\paragraph{Single Layer networks:} We discuss results for FashionMNIST when using classifier $F0$ as model $M$. Figure \ref{fig:metF0Fa} shows as expected that accuracy constantly increases throughout training.  Reconstruction loss remains stable for the first few iterations before decreasing and increasing towards the end. In the light of the information bottleneck theory it was interpreted as the network fitting the data first (leading to a lower reconstruction loss) before compressing, leading to a higher reconstruction loss. We proclaim that first the network moves towards an average of all samples, which can resemble a prototypical class instance. The process of learning an average is well visible in the weight matrices in Figure \ref{fig:weiFa}. The matrices change from being random after initialization matrices (shown in the top row) towards well-recognizable objects, e.g., the first column resembles a T-shirt and the second a pant, before worsening again. Qualitatively this behavior is also shown for reconstructions of $DE$ (see Figure \ref{fig:rec} in Appendix). Towards the end of the training, the ``prototypes'' become less recognizable. Thus, visual recognizability of the weight matrices is aligned with reconstruction loss behavior shown in Figure \ref{fig:metF0Fa}.% The left column in Figure \ref{fig:loClFaSa} illustrates samples that are close to the average.
%But it is more difficult to observe, since a decoder can focus on weights that correlate with the average sample and ignore weights optimized to fit a few samples, as we shall explain. 

Once (the majority of) samples being fairly similar to the average have low loss, weights are adjusted to correctly classify the (few) remaining samples still having large loss. 
Conceptually, one can distinguish three types of inputs $X$ based on the dot product $X\cdot \ov{X}$ of a sample and the (class) average $\ov{X}$: samples $D_S$ with small dot product, samples $D_A$ with ``typical'' (or around average) dot product, and samples $D_B$ with big product. The conceptualization is supported by Figure \ref{fig:diFa} showing the distribution of dot products. Most samples are around the mode, which correspond to samples $D_A$. Samples significantly to the left and right correspond to sets $D_S$ and $D_B$. They are smaller in number.
%Conceptually, one can distinguish three types of inputs $X$ based on the dot product $X\cdot \ov{X}$ of a sample and the (class) average $\ov{X}$: samples $D_S$ with small dot product, samples $D_A$ with ``average'' dot product, and samples $D_B$ with large big product. Samples $D_A$ are samples similar to the average, i.e. $||X-\ov{X}||^2$ is relatively small for $X \in D_A$, while the difference $||X-\ov{X}||^2$ is large for $X \in (D_B \cup D_S)$. The conceptualization is supported by Figure \ref{fig:diFa} showing the distribution of dot products. Most samples are around the mode, which we denote as samples $D_A$. Samples significantly to the left and right correspond to sets $D_S$ and $D_B$. They are smaller in number.
%While the most notable observation might be the skew, we are primarily concerned with the fact that the distribution decays quickly, i.e., there are only a few samples that have large and small deviations from the average dot-product.

Figure \ref{fig:loClFaSa} shows samples $D_A$ (left column) and $D_B$ (right column), which appear brighter and have similar shape to the mean. Samples $D_S$ (middle column) are darker having more diverse (non-typical) shapes. The loss behavior over time is shown in Figure \ref{fig:loClFa} for 1000 samples from these three sets of samples $D_A$, $D_B$ and $D_S$ for multiple classes. It is apparent that samples $D_S$ exhibit largest classifier loss, while those with largest dot product $D_B$ exhibit lowest loss among the three sets. Interestingly, samples in $D_S$ also commonly show an increase of loss initially. This is expected for samples with negative dot product with the mean. Since weights move towards the average initially, small dot product implies small outputs for these samples for the correct class and in turn low probabilities.
Intuitively, one might expect that samples $D_B$ should be classified even better than those close to the average, i.e., $D_A$. However, by looking at the samples in Figure \ref{fig:loClFaSa}, it becomes apparent that a large dot product still allows for many pixels to differ substantially from the class average. For illustration, the majority of gray pixels in $\ov{X}$ are white for $D_B$, but there might still be a considerable number of pixels that differ strongly. The overall shape might even indicate a different class, i.e., some T-Shirts appear as shirts. This is also aligned with the observation that these samples' standard deviation is high.


% \begin{figure}[!htb]
% \centering{
% \centerline{\includegraphics[width=0.4\textwidth]{DistrFash.png}} %\columnwidth
% %\vspace{-12pt}
% \caption{Distribution of the dot product of a sample and the mean, i.e. $X\cdot \ov{X}$. Dot products are standardized for each class.} \label{fig:diFa}}
% \end{figure}
 %That is, assume we are after the first phase yielding that the weights are an average of all samples. For a single weight of a specific class being multiplied with a specific input pixel we can roughly distinguish three situations, 

Fitting to incorrect samples with large deviation from the mean distorts the well-visible ``prototypes'' shown in  Figure \ref{fig:weiFa}. Distorted ``prototypes'' show more contrast and larger differences between adjacent weights. A weight is either very small (black) or very large (white), and neighboring weights often have different signs. To understand the process that leads to higher reconstruction loss, we can view the second phase of learning as fitting to a few high-loss samples.
Assume the pixel average for some position for easy and hard samples is about the same. In this case, the weight will change the same manner for both types of samples, e.g., in Figure \ref{fig:weiFa} a pixel that has become bright due to fitting to easy samples, will become even brighter when fitting to hard samples. Thus, such a pixel helps to more reliably classify easy samples, and it improves the loss of hard samples.
If the average of samples, i.e., $D_A$, differs a lot for a specific pixel from high loss samples $D_S$, in the phase where the loss of $D_A$ is low but still high for $D_S$, the weight is changed considerably, and a black pixel might change to white in this phase and vice versa. 
 
%Generally, matching the average is non-optimal since the average does not aim for being maximally discriminating for classes. It might weigh inputs too much that show low intra-class variance but high inner-class variance thus contributing to noise and potential misclassification. Consider a sweatshirt and pants. The average of both yields a grey shape that is well distinguishable (pants are brighter or darker but most share a fairly common shape, the same holds for sweatshirts). Let us consider the overlap of the average of a pant and a T-shirt. Differences are the middle separating the two legs which is dark for pants and bright for sweatshirts, however, overall much more areas for sweatshirts tend to be dark than for pants, since they are larger, ie. wider. Thus, in tendency a darker sweatshirt is likely to be confused with a pant at this stage. 
%Let $avg(F_j)$ be the average of false samples of $C_j$. Now since samples close to the average are correct, thus their gradient will be small, the updates will move towards the average $avg(F_j)$ where gradients are large. Let's assume that for an input $i$  $avg(F_j)<avg(C_j)$ is large then the weights get decreased compared to the prior phase. If $avg(F_j)~ avg(C_j)$ then the weights are changed about the same otherwise they are increased more strongly.
%In the pants sweatshirt example we have that both pants and sweatshirt share common parts. For both the impact of these common parts is reduced, i.e. it looks closer to a mean grey value. That is the part of the T-shirt covering the upper torso and the area of the pants covering the lower torso become on average darker, while for T-shirts the area where the arms end and for pants parts of the legs also remain. 

\paragraph{Multiple layers and networks:}
Figure \ref{fig:metMuFa} shows the outputs for the last and second last layer for multiple networks for the FashionMNIST dataset. (Additional datasets are in the Appendix). For the last layer, all networks behave qualitatively identically. For the second last layer, the overall pattern remains. For layers closer to the input, it gets weaker. Lower layers are generic, i.e., they are not strongly dependent on the data and even transferable across different datasets. Thus, not surprisingly they are not strongly impacted by a few samples that might differ from the majority but can still be clearly attributed the same dataset.
%However, for VGG we see an initial increase and for $F1$ the change is barely notable.

% \begin{figure}
%   \centering
%   \subfloat[Last Layer]{\includegraphics[width=0.35\textwidth]{Lay0Fash.png} \label{fig:a}} 
%   %\vspace{-12pt}
%   \subfloat[Second last layer]{\includegraphics[width=0.35\textwidth]{Lay1Fash.png} \label{fig:b}} 
%   %\vspace{-6pt}
%   %\subfloat[Third last layer]{\includegraphics[width=0.45\textwidth]{Lay2Fash.png} \label{fig:b}} \\
%   \caption{Normalized accuracy and reconstruction loss for multiple classifiers for the FashionMNIST dataset. Other datasets are in the Appendix.} \label{fig:metMuFa}
%   %\vspace{-12pt}
% \end{figure}













\subsection{Discussion} \label{sec:gen}
\noindent{\textbf{The 3 Phases}:} From the perspective of reconstruction capability, we have identified three phases. An initial phase, where reconstructions are poor, since outputs $o(X)$ are not very informative, i.e., they are based mostly on randomly initialized weights. In the second phase, reconstruction loss decreases and weights move towards class averages. This can also be seen in Eq. \ref{eq:dLy} and \ref{eq:dLy2} showing that the gradient is essentially determined by the majority of samples, i.e., being the mean of the large subsets $C^y_{i-k}$. Thus, initially, with every iteration, i.e., addition of the gradient to the weights, the weights point more and more towards the class mean $\ov{X}$ for $X \in C^y_{i-k}$. 
In the third phase, a few samples can cause a large shift of attribute weights, undoing changes of weights performed in reducing classification loss for the majority of samples. In our analysis for a linear classifier, this means that the classifier does not rely on all possible attributes for the majority of samples but rather focuses on fewer attributes. We have assumed that shift occurs due to the classifier relying on many features towards fewer features, which are also more noisy. This essentially leads to noisier outputs $o(X)$ and, in turn, to poorer reconstruction. One might also assume that all features of a sample $X=(x_i+\epsilon_i)$ are equally noisy and weights $W$ of the linear classifier become less uniform, which in turn increases the variance of $S_{y,\ep}$ and, thus, eventually the reconstruction error as we discuss more in the Appendix.
%Add Appendix: That is, after a few iterations weights are fairly similar in magnitude, however, once the fitting to the ``few'' samples occurs, some weights increase in magnitude, while others increase less and eventually decrease. This leads to different magnitudes of weights. Thus, the variance of $S_{y,\ep}:=\sum_{i \in A_y} w_i\epsilon_i$ increases and, in turn, the ratio $(S_{y,\ep}/S_y)^2$ being part of the reconstruction loss.

\noindent{\textbf{The loss function as the driver of the phases}:} While empirically we have shown that the three phases of the reconstruction loss can occur for multiple datasets, networks and layers, they are most notable for the last layer of a network. Features in the last layer are the least shared among classes, since the SoftMax layer paired with the cross-entropy loss of the classifier enforces discriminative features, i.e., features that strongly correlated with one or few classes only. That is, during training outputs of the last linear layer become more and more discriminative, thereby, forgoing information on the appearance of a sample. For illustration, for a classifier distinguishing cars, trucks and flowers (among other classes), for a car resembling some similarities with a truck, in early phases of the training the outputs $o_y$ for each class might be in a similar order of magnitude say $(0.6,0.3,0.01,..)$ for the three classes. However, as the classifier becomes more discriminative, it pushes, ideally, one to infinity and the other to negative infinity, i.e., towards $(\infty,-\infty,-\infty,...)$. The Softmax also reduces the nuanced differences between classes. Thus, information content on the appearance is lost due to becoming more discriminative. This effect of the SoftMax layer is most profound in the last layer and is less pronounced in lower layers. This has also been observed in \cite{saxe19} using mutual information through simulation rather than mathematical proofs.

\noindent{\textbf{Classification vs. Reconstruction over time:}}
Comparing training accuracy and reconstruction loss across training, we see that both share the first two phases, i.e., training accuracy might also be barely changing in the first few iterations before it increases. However, once training accuracy has reached a high level, indicating that both samples are well fit, we can observe that reconstruction loss increases due to fitting to a few.


\noindent{\textbf{Model assumptions}:}
In our model, we assumed that features are not shared among classes. However, one might wonder what happens if some input features are indicative of multiple classes. Say 1/2 of all features are indicative of $\log l$ classes and the other of just 1. Such features are effectively discouraged in the optimization process, since they increase the output $o_y$ of multiple classes,  they inc the denominator.

The size of the small subset, given by parameter $k$, determines when the fitting to the small subset occurs. That is, for very small $k$, the majority of samples will be fitted almost perfectly before the change to the small subset occurs. If $k$ is large, i.e., moving towards 1/2, the fitting occurs earlier, i.e., when the majority of samples are not yet fit well.

All attributes noisy?

Attributes shared?



\section{Related Work}
The information bottleneck~\citep{tish00} was used for analysis of deep learning in~\citep{tish15,tish17}. It suggests a principled way to ``find a maximally compressed mapping of the input variable that preserves as much as possible the information on the output variable''~\citep{tish17}. To this end, layers $h_i$ of a network are viewed as a Markov chain for which holds given $i\geq j$ using the data processing inequality: $$I(Y;X) \geq I(Y;h_j) \geq I(Y;h_i) \geq I(Y;\hat{Y})$$ 
Learning is seen as the process that maximizes $I(Y;h_i)$ while minimizing $I(h_{i-1};h_i)$, where the latter can be interpreted as the minimal description length of the layer. In our view, we agree on the former (at least on a qualitative level), but we do not see minimizing the description length as a goal of learning. In our perspective and also in our framework, it can be a consequence of the first objective, i.e. to discriminate among classes, and existing learning algorithms, i.e., gradient descent. From a generalization perspective, it seems preferable to cling onto even the smallest bit of information of the input $X$, even if its highly redundant and, as long as it \emph{could} be useful for classification. This statement is also supported by~\citep{saxe19} who show that compression is not necessary for generalization behavior and that fitting and compression happen in parallel rather than sequentially. A recent review~\citep{gei21} also concludes that the absence of compression is more likely to hold. This is aligned with our findings, since in our analysis, ``information loss'' on the input is a consequence of weighing input attributes too much that are sensitive to additive noise. In contrast to our work, their analysis is within the IB framework. Still, it remedies an assumption of~\citep{tish17}. Namely,~\citep{saxe19} investigates different non-linearities, i.e., the more common ReLU activations rather than sigmoid activations. Recently,~\citep{lor21} argues that compression is only observed consistently in the output layer. The IB framework has also been used to show that neural networks must lose information~\citep{liu20} irrespective of the data it is trained on. From our perspective the alleged information loss measured in terms of the reconstruction capability could be minimal at best. In particular, it is evident that at least initially reconstruction is almost perfect for wide networks following theory on random projections, i.e., the Johnson-Lindenstrauss Lemma~\citep{joh84} proved that random projections allow embedding $n$ points into an $O(\log n/\epsilon^2)$ dimensional space while preserving distances within a factor of $1\pm \epsilon$. This bound is also tight according to~\citep{lar17} and it can be extended to cases where we apply non-linearities, i.e., $ReLU$. \\
In~\citep{wang21pac} an information measure based on weights is used to show empirically that fitting and compression phase exist. In~\citep{ach18} also two phases were suggested based on empirical analysis. The call the second phase ``forgetting''.
Across all these works, our view is not contradictory to the notion of ``forgetting'' or ``compression'' but we go one step further saying that the network ``forgets'' about the majority to fit a few samples.
\\
%Thus, to set minimization of information flow between layers as an objective is not necessarily beneficial, e.g., in case we should learn the identity mapping $X=Y$ then $I(h_{i-1};h_i)$ should obviously be maximized.
~\citep{gei21} also discussed the idea of geometric compression based on prior works on IB analysis. However, the literature was inconclusive according to~\citep{gei21} on whether compression occurs due to scaling or clustering. Our analysis is inherently geometry (rather than information) focused, i.e., we measure learning based on how well classes can be separated using linear separators in learnt latent spaces. That is, our work favors class-specific clustering as set forth briefly in~\citep{gol18}, but we derive it not using the IB framework.\\\citep{ala17} used a single linear layer to analyze networks empirically. However, their focus was to understand the suitability of intermediate layers for classification rather than learning dynamics.\\
As the IB has also been applied to other types of tasks, i.e., autoencoding~\citep{tap20}, we believe that our approach might also be extended to such tasks.\\

The idea to reconstruct inputs from layer activations has been outlined in the context of explainability~\citep{sch21cla}. The idea is to compare reconstructions using a decoder with original inputs to assess what information (or concepts) are ``maintained'' in a model. Our work also touches upon linear decoders that have been studied extensively, e.g.,~\citep{kun19}. It also estimates reconstruction errors from noisy inputs $x_i+\epsilon$~\citep{car09}.

%Our work also uses theory on random projections, which have commonly been used in the context of clustering~\citep{sch17,sch14}. In these (and many other) applications random projections remain unaltered and are used for dimensionality reduction. In particular, the Johnson-Lindenstrauss Lemma~\citep{joh84} proved that random projections allow to embed $n$ points into an $O(\log n/\epsilon^2)$ dimensional space while preserving distances within a factor of $1\pm \epsilon$. This bound is also tight according to~\citep{lar17}.

% VERY SIMILAR: {ma2019} Quantifying layerwise information discarding of neural networks

%i-REVNET: DEEP INVERTIBLE NETWORKS, https://arxiv.org/abs/1802.07088)
%The Information Bottleneck Problem and Its     Applications in Machine Learning
%Nonlinear Information Bottleneck
%Where is the Information in a Deep Neural Network?
%Understanding convolutional neural networks with information theory: An initial exploration
%Why should we add early exits to neural networks?
%Evaluating representations by the complexity of learning low-loss predictors
%Are Deep Neural Architectures Losing Information? Invertibility Is Indispensable
%What Information Does a ResNet Compress?
%Information bottleneck theory on convolutional neural networks 2021
%Good Explanation and Refs: Wikipedia - Information bottleneck method\\
%Good explanation: https://arnavkansal.com/dl/2018/05/01/Information-Theory-for-Deep-Learning/
%Good Explanation: https://www.quora.com/How-is-the-information-bottleneck-theory-of-deep-learning-different-from-the-known-example-of-having-a-reduced-dimension-hidden-layer-in-an-autoencoder
%Learning Without Feedback: Fixed Random Learning Signals Allow for Feedforward Training of Deep Neural Networks
%https://github.com/stevenliuyi/information-bottleneck


\section{Conclusions}
Theory of deep learning is limited. This work focused on a very pressing problem, i.e., understanding the learning process. To this end, it rigorously analyzed a simple dataset modeling many observations of common datasets. Our results highlight that few samples are likely to profoundly impact weights in later stages of the training, potentially compromising classifier robustness.



